Towards Predicting Equilibrium Distributions for Molecular Systems with Deep Learning

Advances in deep learning have greatly improved structure prediction of molecules. However, many macroscopic observations that are important for real-world applications are not functions of a single molecular structure, but rather determined from the equilibrium distribution of structures. Traditional methods for obtaining these distributions, such as molecular dynamics simulation, are computationally expensive and often intractable. In this paper, we introduce a novel deep learning framework, called Distributional Graphormer (DiG), in an attempt to predict the equilibrium distribution of molecular systems. Inspired by the annealing process in thermodynamics, DiG employs deep neural networks to transform a simple distribution towards the equilibrium distribution, conditioned on a descriptor of a molecular system, such as a chemical graph or a protein sequence. This framework enables efficient generation of diverse conformations and provides estimations of state densities. We demonstrate the performance of DiG on several molecular tasks, including protein conformation sampling, ligand structure sampling, catalyst-adsorbate sampling, and property-guided structure generation. DiG presents a significant advancement in methodology for statistically understanding molecular systems, opening up new research opportunities in molecular science.

==> tables/protein_ligand_feature_list.tex <==
\begin{table}[t]
\centering
\small
{
\caption{\textbf{Feature list of protein-ligand models.}} Each feature listed below could be obtained by RDKit [REF:RDKIT].
}\label{tab:protein_ligand_feature_list}
\begin{tabular}{l|l|l}
    \toprule
    Category & Feature & RDKit method \\
    \midrule
    Atom feature &
  atomic num & GetAtomicNum() \\
& chirality & GetChiralTag() \\
& degree & GetTotalDegree() \\
& formal charge & GetFormalCharge() \\
& number of Hydrogens & GetTotalNumHs() \\
& number of radical electrons & GetNumRadicalElectrons() \\
& hybridization type & GetHybridization() \\
& is aromatic & GetIsAromatic() \\
& is in a ring & IsInRing() \\
    \midrule
    Bond feature &
  bond type     & GetBondType() \\
& bond stereo   & GetStereo() \\
& is conjugated & GetIsConjugated() \\
    \midrule
    Protein edge feature & 
    is atom within cutoff 5\AA & - \\
    \bottomrule
\end{tabular}

\end{table}
